Low-Dimensional Hyperbolic Knowledge Graph Embeddings

Knowledge graph (KG) embeddings learn low-dimensional representations of entities and relations to predict missing facts. KGs often exhibit hierarchical and logical patterns which must be preserved in the embedding space. For hierarchical data, hyperbolic embedding methods have shown promise for high-fidelity and parsimonious representations. However, existing hyperbolic embedding methods do not account for the rich logical patterns in KGs. In this work, we introduce a class of hyperbolic KG embedding models that simultaneously capture hierarchical and logical patterns. Our approach combines hyperbolic reflections and rotations with attention to model complex relational patterns. Experimental results on standard KG benchmarks show that our method improves over previous Euclidean- and hyperbolic-based efforts by up to 6.1% in mean reciprocal rank (MRR) in low dimensions. Furthermore, we observe that different geometric transformations capture different types of relations while attention-based transformations generalize to multiple relations. In high dimensions, our approach yields new state-of-the-art MRRs of 49.6% on WN18RR and 57.7% on YAGO3-10.

==> model/optimization.tex <==
Optimization in hyperbolic space normally requires Riemannian Stochastic Gradient Descent (RSGD) \cite{bonnabel2013stochastic}, as was used in MuRP. 
RSGD is challenging in practice. 
Instead, we define all the \model{} parameters in the tangent space at the origin (our parameter space), optimize embeddings using standard Euclidean techniques, and use the exponential map to recover the hyperbolic parameters.

Concretely, \model{} optimizes the entity and relationship embeddings $(\mathbf{e}^E_v)_{v\in\mathcal{V}}$ and $(\mathbf{r}^E_r)_{r\in\mathcal{R}}$, which are mapped to the Poincar\'e ball with:
\begin{equation}
    \mathbf{e}_v^H=\mathrm{exp}_\mathbf{0}^{c_r}(\mathbf{e}_v^E)  \ \ \text{and}\ \
    \mathbf{r}_r^H=\mathrm{exp}_\mathbf{0}^{c_r}(\mathbf{r}_r^E),\label{eq:mapping}
\end{equation}
where $c_r=\mathrm{Softplus}(c_r')\in\mathbb{R}_+$ is a learned relation-specific absolute hyperbolic curvature, providing more flexibility to the model, about whether to embed relations into a more curved hyperbolic space (more ``tree-like"), or into an Euclidean geometry ($c_r\rightarrow 0$).  
As we shall see in the Section \ref{subsec:high_dim}, trainable curvature is is critical to avoid precision round-off errors in high dimensions. 

The model parameters are then $\{(\Theta_r, \Phi_r, \mathbf{r}_r^E, \mathbf{a}_r, c_r)_{r\in\mathcal{R}},(\mathbf{e}_v^E, b_v)_{v\in\mathcal{V}}\}$, which are all Euclidean parameters and can be learned using standard Euclidean optimization techniques. 
We train \model{} by minimizing the full cross-entropy loss where negative examples for a true triple $(h, r, t)$ are all triples obtained by perturbing the tail entity:
\begin{align}\label{eq:loss}
    \mathcal{L}=\sum\limits_{t'\in\mathcal{V}}\mathrm{log}(1 +& \mathrm{exp}(y_{t'}s(h,r,t'))),\\
    \mathrm{where}\ \ y_{t'}&=\begin{cases}-1 & \mathrm{if}\ \  t'=t\\
    1 & \mathrm{otherwise.}
    \end{cases}
\end{align}
